PyOcto: A high-throughput seismic phase associator

Seismic phase association is an essential task for characterising seismicity: given a collection of phase picks, identify all seismic events in the data. In recent years, machine learning pickers have lead to a rapid growth in the number of seismic phase picks. Even though new associators have been suggested, these suffer from long runtimes and sensitivity issues when faced with dense seismic sequences. Here we introduce PyOcto, a novel phase associator tackling these issues. PyOcto uses 4D space-time partitioning and can employ homogeneous and 1D velocity models. We benchmark PyOcto against popular state of the art associators on two synthetic scenarios and a real, dense aftershock sequence. PyOcto consistently achieves detection sensitivities on par or above current algorithms. Furthermore, its runtime is consistently at least 10 times lower, with many scenarios reaching speedup factors above 50. On the challenging 2014 Iquique earthquake sequence, PyOcto achieves excellent detection capability while maintaining a speedup factor of at least 70 against the other models. PyOcto is available as an open source tool for Python on Github and through PyPI.

==> tables/full_benchmark.tex <==
\begin{longtable}{lrrlrrrrrr}
\caption{Full results of synthetic benchmark. We abbreviate \textit{picks per event} as \textit{ppe}.} \label{tab:full_benchmark} \\
\toprule
Scenario & Events & Noise & Associator & Precision & Recall & F1 & Missing ppe & Additional ppe & Run time [s] \\
\midrule
\endfirsthead
\caption[]{Full results of synthetic benchmark. We abbreviate \textit{picks per event} as \textit{ppe}.} \\
\toprule
Scenario & Events & Noise & Associator & Precision & Recall & F1 & Missing ppe & Additional ppe & Run time [s] \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
shallow & 100 & 0.30 & Gamma & 1.00 & 0.99 & 0.99 & 0.08 & 0.04 & 5.04 \\
shallow & 100 & 0.30 & PyOcto & 1.00 & 0.96 & 0.98 & 0.06 & 0.03 & 0.74 \\
shallow & 100 & 0.30 & PyOcto1D & 1.00 & 0.96 & 0.98 & 0.04 & 0.03 & 1.52 \\
shallow & 100 & 0.30 & REAL & 0.99 & 0.93 & 0.96 & 2.16 & 0.01 & 10.11 \\
shallow & 100 & 0.30 & REAL1D & 1.00 & 0.93 & 0.96 & 5.91 & 0.00 & 11.52 \\
shallow & 100 & 1.00 & Gamma & 1.00 & 0.97 & 0.98 & 0.07 & 0.21 & 14.93 \\
shallow & 100 & 1.00 & PyOcto & 1.00 & 0.96 & 0.98 & 0.28 & 0.21 & 1.15 \\
shallow & 100 & 1.00 & PyOcto1D & 1.00 & 0.96 & 0.98 & 0.23 & 0.16 & 1.54 \\
shallow & 100 & 1.00 & REAL & 0.98 & 0.93 & 0.95 & 2.86 & 0.08 & 22.86 \\
shallow & 100 & 3.00 & Gamma & 0.97 & 0.86 & 0.91 & 0.17 & 0.59 & 120.52 \\
shallow & 100 & 3.00 & PyOcto & 1.00 & 0.96 & 0.98 & 0.47 & 0.68 & 1.69 \\
shallow & 100 & 3.00 & PyOcto1D & 1.00 & 0.96 & 0.98 & 0.41 & 0.55 & 2.11 \\
shallow & 100 & 3.00 & REAL & 0.99 & 0.96 & 0.97 & 3.20 & 0.41 & 59.62 \\
shallow & 100 & 3.00 & REAL1D & 0.95 & 0.91 & 0.93 & 8.90 & 0.42 & 64.44 \\
shallow & 500 & 0.30 & Gamma & 0.98 & 0.92 & 0.95 & 0.34 & 0.37 & 126.18 \\
shallow & 500 & 0.30 & PyOcto & 1.00 & 0.93 & 0.96 & 0.68 & 0.52 & 4.47 \\
shallow & 500 & 0.30 & PyOcto1D & 1.00 & 0.93 & 0.97 & 0.61 & 0.42 & 5.37 \\
shallow & 500 & 0.30 & REAL & 0.99 & 0.93 & 0.96 & 3.07 & 0.33 & 64.30 \\
shallow & 500 & 0.30 & REAL1D & 0.95 & 0.84 & 0.89 & 7.55 & 0.33 & 71.81 \\
shallow & 500 & 1.00 & Gamma & 0.93 & 0.85 & 0.89 & 0.39 & 1.02 & 2967.45 \\
shallow & 500 & 1.00 & PyOcto & 1.00 & 0.95 & 0.97 & 0.69 & 1.07 & 5.17 \\
shallow & 500 & 1.00 & PyOcto1D & 1.00 & 0.95 & 0.97 & 0.63 & 0.76 & 5.95 \\
shallow & 500 & 1.00 & REAL & 1.00 & 0.96 & 0.98 & 2.88 & 0.64 & 120.98 \\
shallow & 500 & 1.00 & REAL1D & 0.96 & 0.87 & 0.91 & 7.65 & 0.62 & 132.69 \\
shallow & 500 & 3.00 & PyOcto & 1.00 & 0.94 & 0.97 & 1.04 & 3.17 & 7.75 \\
shallow & 500 & 3.00 & PyOcto1D & 1.00 & 0.94 & 0.97 & 0.93 & 2.38 & 8.63 \\
shallow & 500 & 3.00 & REAL & 0.99 & 0.92 & 0.96 & 3.14 & 1.79 & 280.00 \\
shallow & 500 & 3.00 & REAL1D & 0.95 & 0.85 & 0.90 & 6.94 & 1.86 & 304.51 \\
shallow & 2000 & 0.30 & PyOcto & 0.99 & 0.88 & 0.93 & 1.85 & 2.31 & 21.37 \\
shallow & 2000 & 0.30 & PyOcto1D & 0.99 & 0.89 & 0.94 & 1.53 & 1.77 & 24.98 \\
shallow & 2000 & 0.30 & REAL & 0.99 & 0.87 & 0.93 & 3.96 & 1.53 & 293.98 \\
shallow & 2000 & 0.30 & REAL1D & 0.93 & 0.78 & 0.85 & 8.24 & 1.68 & 315.48 \\
shallow & 2000 & 1.00 & PyOcto & 0.98 & 0.87 & 0.92 & 2.27 & 4.88 & 25.85 \\
shallow & 2000 & 1.00 & PyOcto1D & 0.99 & 0.89 & 0.94 & 1.82 & 3.69 & 29.22 \\
shallow & 2000 & 1.00 & REAL & 0.99 & 0.88 & 0.93 & 4.27 & 3.03 & 541.86 \\
shallow & 2000 & 1.00 & REAL1D & 0.94 & 0.77 & 0.85 & 8.36 & 3.12 & 570.99 \\
shallow & 2000 & 3.00 & PyOcto & 0.65 & 0.70 & 0.67 & 3.81 & 11.81 & 118.86 \\
shallow & 2000 & 3.00 & PyOcto1D & 0.85 & 0.81 & 0.83 & 3.00 & 9.18 & 118.70 \\
shallow & 2000 & 3.00 & REAL & 0.90 & 0.79 & 0.84 & 5.33 & 7.17 & 1247.50 \\
shallow & 2000 & 3.00 & REAL1D & 0.80 & 0.68 & 0.74 & 9.55 & 7.39 & 1293.43 \\
subduction & 100 & 0.30 & Gamma & 0.98 & 0.97 & 0.97 & 3.18 & 0.02 & 5.50 \\
subduction & 100 & 0.30 & PyOcto & 1.00 & 0.99 & 0.99 & 3.22 & 0.07 & 0.44 \\
subduction & 100 & 0.30 & PyOcto1D & 1.00 & 0.98 & 0.99 & 0.32 & 0.05 & 1.34 \\
subduction & 100 & 0.30 & REAL & 1.00 & 0.97 & 0.98 & 2.36 & 0.10 & 149.07 \\
subduction & 100 & 0.30 & REAL1D & 1.00 & 0.97 & 0.98 & 0.94 & 0.08 & 155.14 \\
subduction & 100 & 1.00 & Gamma & 0.94 & 0.95 & 0.95 & 3.48 & 0.06 & 7.31 \\
subduction & 100 & 1.00 & PyOcto & 0.99 & 0.98 & 0.98 & 3.24 & 0.14 & 1.45 \\
subduction & 100 & 1.00 & PyOcto1D & 1.00 & 0.98 & 0.99 & 0.44 & 0.12 & 0.80 \\
subduction & 100 & 1.00 & REAL & 0.99 & 0.98 & 0.98 & 2.73 & 0.14 & 282.84 \\
subduction & 100 & 1.00 & REAL1D & 1.00 & 0.98 & 0.99 & 1.16 & 0.32 & 322.51 \\
subduction & 100 & 3.00 & Gamma & 0.98 & 0.94 & 0.96 & 3.61 & 0.28 & 7.73 \\
subduction & 100 & 3.00 & PyOcto & 1.00 & 0.99 & 0.99 & 3.02 & 0.33 & 7.87 \\
subduction & 100 & 3.00 & PyOcto1D & 1.00 & 0.98 & 0.99 & 0.41 & 0.23 & 6.78 \\
subduction & 100 & 3.00 & REAL & 1.00 & 0.96 & 0.98 & 2.32 & 0.33 & 633.18 \\
subduction & 100 & 3.00 & REAL1D & 1.00 & 0.99 & 0.99 & 1.09 & 0.41 & 807.16 \\
subduction & 500 & 0.30 & Gamma & 0.90 & 0.83 & 0.87 & 3.84 & 0.31 & 65.93 \\
subduction & 500 & 0.30 & PyOcto & 0.97 & 0.94 & 0.95 & 3.57 & 0.35 & 29.65 \\
subduction & 500 & 0.30 & PyOcto1D & 1.00 & 0.97 & 0.98 & 0.61 & 0.27 & 11.59 \\
subduction & 500 & 0.30 & REAL & 0.99 & 0.92 & 0.95 & 3.13 & 0.44 & 781.53 \\
subduction & 500 & 0.30 & REAL1D & 0.99 & 0.93 & 0.96 & 1.38 & 0.55 & 861.39 \\
subduction & 500 & 1.00 & Gamma & 0.78 & 0.70 & 0.74 & 3.91 & 0.64 & 115.60 \\
subduction & 500 & 1.00 & PyOcto & 0.96 & 0.92 & 0.94 & 3.73 & 0.70 & 40.84 \\
subduction & 500 & 1.00 & PyOcto1D & 0.99 & 0.96 & 0.98 & 0.74 & 0.56 & 39.70 \\
subduction & 500 & 1.00 & REAL & 0.98 & 0.90 & 0.93 & 3.19 & 0.79 & 1480.71 \\
subduction & 500 & 1.00 & REAL1D & 0.98 & 0.91 & 0.94 & 1.57 & 1.13 & 1803.82 \\
subduction & 500 & 3.00 & Gamma & 0.61 & 0.47 & 0.53 & 4.51 & 1.62 & 11758.45 \\
subduction & 500 & 3.00 & PyOcto & 0.95 & 0.93 & 0.94 & 3.66 & 1.55 & 21.26 \\
subduction & 500 & 3.00 & PyOcto1D & 0.99 & 0.98 & 0.99 & 1.00 & 1.09 & 7.56 \\
subduction & 500 & 3.00 & REAL & 0.97 & 0.90 & 0.93 & 3.29 & 1.55 & 3467.77 \\
subduction & 500 & 3.00 & REAL1D & 0.98 & 0.94 & 0.96 & 2.08 & 2.26 & 4470.67 \\
subduction & 2000 & 0.30 & Gamma & 0.54 & 0.43 & 0.48 & 4.85 & 1.38 & 2842.45 \\
subduction & 2000 & 0.30 & PyOcto & 0.89 & 0.81 & 0.85 & 4.51 & 1.45 & 109.50 \\
subduction & 2000 & 0.30 & PyOcto1D & 0.98 & 0.89 & 0.93 & 1.48 & 0.98 & 93.24 \\
subduction & 2000 & 0.30 & REAL & 0.92 & 0.72 & 0.80 & 4.21 & 1.56 & 3210.97 \\
subduction & 2000 & 0.30 & REAL1D & 0.97 & 0.78 & 0.87 & 2.60 & 2.00 & 3574.75 \\
subduction & 2000 & 1.00 & PyOcto & 0.83 & 0.77 & 0.80 & 4.51 & 2.46 & 176.07 \\
subduction & 2000 & 1.00 & PyOcto1D & 0.96 & 0.89 & 0.92 & 1.90 & 1.83 & 146.68 \\
subduction & 2000 & 1.00 & REAL & 0.89 & 0.70 & 0.78 & 4.54 & 2.73 & 5571.98 \\
subduction & 2000 & 1.00 & REAL1D & 0.93 & 0.76 & 0.84 & 3.34 & 3.42 & 6602.46 \\
subduction & 2000 & 3.00 & PyOcto & 0.27 & 0.51 & 0.36 & 5.74 & 5.47 & 636.98 \\
subduction & 2000 & 3.00 & PyOcto1D & 0.46 & 0.74 & 0.57 & 3.35 & 4.20 & 679.37 \\
subduction & 2000 & 3.00 & REAL & 0.43 & 0.43 & 0.43 & 5.87 & 5.70 & 9675.44 \\
subduction & 2000 & 3.00 & REAL1D & 0.51 & 0.54 & 0.53 & 5.02 & 6.57 & 11269.04 \\
\end{longtable}


==> tables/params_gamma.tex <==
\begin{table}[ht!]
\caption{Parameters for the GaMMA associator. All parameters not provided in the table were used at their default values. The parameters for the application to the Iquique sequence are identical to the \textit{Subduction} parameters. Where possible, we use the parameter name from the published implementation. We omit purely functional parameters.}
\label{tab:params_gamma}
\centering
\begin{tabular}{lll}
\toprule
Parameter & Shallow & Subduction \\
\midrule
ncpu & 15 & 15 \\
x(km) & [395, 605] & [250, 600] \\
y(km) & [7560, 7790] & [7200, 8000] \\
z(km) & [0, 30] & [0, 250] \\
p velocity & 6.3 & 7.0 \\
s velocity & 3.7 & 4.0 \\
use\_dbscan & True & True \\
use\_amplitude & False & False \\
method & BGMM & BGMM \\
oversample\_factor & 4 & 4 \\
dbscan\_eps & 25 & 25 \\
dbscan\_min\_samples & 3 & 3 \\
min\_picks\_per\_eq & 10 & 10 \\
max\_sigma11 & 2.0 & 2.0 \\
max\_sigma22 & 1.0 & 1.0 \\
max\_sigma12 & 1.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/params_pyocto.tex <==
\begin{table}[ht!]
\caption{Parameters for the PyOcto associator. All parameters not provided in the table were used at their default values. The parameters for the application to the Iquique sequence are identical to the \textit{Subduction} parameters. Where possible, we use the parameter name from the published implementation. We omit purely functional parameters. If two values are provided, the first is for the homogeneous velocity model, the second for the 1D model.}
\label{tab:params_pyocto}
\centering
\begin{tabular}{lll}
\toprule
Parameter & Shallow & Subduction \\
\midrule
xlim & [395., 605.] & [250., 600.]\\
ylim & [7560., 7790.] & [7200., 8000.]\\
zlim & [0., 30.] & [0., 250.]\\
time\_before & 300. & 300\\
n\_picks & 10 & 10\\
n\_p\_and\_s\_picks & 4 & 4\\
pick\_match\_tolerance & 2 / 1.5 & 2 / 1.5\\
p\_velocity & 6.3 & 7.0\\
s\_velocity & 3.7 & 4.0\\
velocity\_model tolerance & 2 / 1.5 & 2 / 1.5\\
velocity\_model association\_cutoff\_distance & 100 & 250 \\

\bottomrule
\end{tabular}
\end{table}


==> tables/params_real.tex <==
\begin{table}[ht!]
\caption{Parameters for the REAL associator. All parameters not provided in the table were used at their default values. The parameters for the application to the Iquique sequence are identical to the \textit{Subduction} parameters. We omit purely functional parameters. Note that some parameters are only used in the homogeneous (velocities) or in the 1D model (traveltime grid details).}
\label{tab:params_real}
\centering
\begin{tabular}{lll}
\toprule
Parameter & Shallow & Subduction \\
\midrule
search\_range\_horizontal\_deg & 0.2 & 1.0\\
search\_range\_vertical\_km & 30 & 250\\
grid\_size\_horizontal\_deg & 0.04 & 0.1\\
grid\_size\_vertical\_km & 3 & 10\\
vp & 6.3 & 7.0\\
vs & 3.7 & 4.0\\

shallow\_vp & 5.3 & 5.3\\
shallow\_vs & 3.1 & 3.1\\
elevation\_correction & False & True\\

tt\_range\_horizontal\_deg & 3 & 6\\
tt\_grid\_size\_horizontal\_deg & 0.04 & 0.05\\
tt\_grid\_size\_vertical\_km & 3 & 3\\

\bottomrule
\end{tabular}
\end{table}

